Impossibilities for Obviously Strategy-Proof Mechanisms

We explore the approximation power of deterministic obviously strategy-proof mechanisms in auctions, where the objective is welfare maximization. A trivial ascending auction on the grand bundle guarantees an approximation of $\min\{m,n\}$ for all valuation classes, where $m$ is the number of items and $n$ is the number of bidders. We focus on two classes of valuations considered "simple": additive valuations and unit-demand valuations. For additive valuations, Bade and Gonczarowski [EC'17] have shown that exact welfare maximization is impossible. No impossibilities are known for unit-demand valuations. We show that if bidders' valuations are additive or unit-demand, then no obviously strategy-proof mechanism gives an approximation better than $\min\{m,n\}$. Thus, the aforementioned trivial ascending auction on the grand bundle is the optimal obviously strategy-proof mechanism. These results illustrate a stark separation between the power of dominant-strategy and obviously strategy-proof mechanisms. The reason for it is that for both of these classes the dominant-strategy VCG mechanism does not only optimize the welfare exactly, but is also "easy" both from a computation and communication perspective. In addition, we prove tight impossibilities for unknown single-minded bidders in a multi-unit auction and in a combinatorial auction. We show that in these environments as well, a trivial ascending auction on the grand bundle is optimal.

==> app-sec-sm.tex <==
\section{An Impossibility for a Combinatorial Auction with Unknown Single-Minded Bidders}\label{app-sec-sm}
%\toedit{We remind that there exists a mechanism that achieves an approximation of $k$ to the optimal welfare for unknown single-minded bidders, if the largest set desired is of size $k$.} 
In this section, we consider unknown single-minded bidders in a combinatorial auction.   
% The valuation of each player $i$ is specified by $v_i:[m]\to \mathbb{R}$.  
The definition of 
unknown single-minded bidders is as follows:  a valuation $v_i$ is \emph{single-minded} if it is parameterized with a bundle $S^\ast$ and a value $x$ such that:
$$
v_i^{x,S^\ast}(S)=\begin{cases}
    x \quad S^\ast\subseteq  S, \\
    0 \quad \text{otherwise.}
\end{cases}
$$
We show an impossibility result for a domain that has valuations that are  parameterized with different desired bundles, so the bidders are \emph{unknown single-minded}. Domains in which the bundle parameter of all valuations is fixed are called \emph{known singe-minded}.   



% \begin{theorem}
% A multi-unit auction with $m\ge 2$ items and $n\ge 2$ unknown-single minded bidders has  no
%  obviously strategy-proof, individually rational and no-negative-transfers mechanism  that gives approximation strictly  better than  $\min\{n,m\}$ to the social welfare.  
% \end{theorem}
\subsection{Proof of Theorem \ref{cor-ca-sm}}
Fix an auction with a set of items  $M$ and $n$ bidders. 
Denote the elements in the set of items with $\{e_1,\ldots,e_m\}$. 
We assume that the domain $V_i$ of each bidder consists of single minded valuations with values in  $\{0,1,\ldots,poly(m,n)\}$.
Assume towards a contradiction that 
there exists an obviously strategy-proof, individually rational, no-negative-transfers mechanism $\mathcal M$ together with strategy profile $\mathcal S=(\mathcal S_1,\ldots,\mathcal S_n)$
that implement an allocation rule and payment schemes  $(f,P_1,\ldots,P_n):V_1\times\cdots\times V_n\to\mathcal T\times \mathbb R^n$, where $f$ 
gives approximation ratio strictly better than $\min\{m,n\}$ to the social welfare.  

% Thus, there exists
% an allocation rule
% $f:V_1\times\cdots\times V_n\to \mathcal T$  and payment schemes  $P_1,\ldots,P_n:V_1\times \cdots \times V_n\to \mathbb{R}^n$ the payment schemes  

% Fix an allocation rule  with approximation ratio $\alpha$ such that $\alpha>\max\{\frac{1}{n},\frac{1}{m}\}$. Let $\mathcal{M}$ be a normalized mechanism 
% and strategies  $(\mathcal S_1,\ldots,\mathcal{S}_n)$  that realize $f$ together with the payment schemes $P_1,\ldots,P_n:V_1\times \cdots \times V_n\to \mathbb{R}^n$. 

We start by defining several valuations. For each player $i\le m$, we define:
$$
v_i^{one}(S)=\begin{cases}
1 \quad e_i\in S, \\
0 \quad \text{otherwise.}
\end{cases}
$$
For each player $i>m$, we set:
$$
v_i^{one}(S)=\begin{cases}
1 \quad e_m\in S, \\
0 \quad \text{otherwise.}
\end{cases}
$$
Observe that given the valuation profile $(v_1^{one},\ldots,v_n^{one})$, there are at least two bidders such that $f$ assigns to them at least one item
because of its approximation guarantee.  
% The reason for it is that the optimal welfare given $(v_1^{one},\ldots,v_n^{one})$  is $\min\{m,n\}$. Since $f$ guarantees strictly more than $\max\{\frac{1}{m},\frac{1}{n}\}$ of the welfare, the welfare has to be strictly larger than $1$. 
Without loss of generality, we assume that bidders $1$ and $2$ are allocated at least one item each. 
We now define two additional valuations for bidders $1$ and $2$:
$$
v_1^{all}(S)=\begin{cases}
K^4 \quad S=M, \\
0 \quad \text{otherwise.}
\end{cases} \\\quad 
v_1^{ONE}(S)= \begin{cases}
1 \quad e_1\in S, \\
0 \quad \text{otherwise.}
\end{cases}
$$
$$
v_2^{all}(S)=\begin{cases}
K^4 \quad S=M, \\
0 \quad \text{otherwise.}
\end{cases} \\\quad 
v_2^{ONE}(S)= \begin{cases}
1 \quad e_2\in S, \\
0 \quad \text{otherwise.}
\end{cases}
$$
where $K=\max\{m,n\}$. 
% We now show that the mechanism and the strategies $(\mathcal S_1,\ldots,\mathcal S_n)$ do not realize $f$ in obviously dominant strategies. 
For the analysis of the mechanism, we define the following subsets of the domains of the valuations:
$
\mathcal{V}_1=\{v_1^{one},v_1^{ONE},v_1^{all}\}$,  $\mathcal{V}_2=\{v_2^{one},v_2^{ONE},v_2^{all}\}$ and for every player $i\ge 3$, we set $\mathcal{V}_i=\{v_i^{one}\}$. We use the notation $\mathcal V=\mathcal{V}_1\times\cdots\times \mathcal{V}_n$. The rest of the proof is identical to the proof of Theorem \ref{thm-lb-mua}. 


==> characterization.tex <==
\subsection{Generalized Ascending Auctions}
We begin by making some basic definitions that we will be of use when analyzing mechanisms, which are very similar to the ones in \cite{DRV22}. 
\src{Maybe write here more about the tree? What I mean by it? Maybe add a drawing?}
\begin{definition}
	Fix some player $i$ and vertex $u$ where player $i$ speaks. The \emph{minimal price} of bundle $S$ at vertex $u$ for player $i$  is $p_S$ if $p_S$ is the minimal payment of player $i$ among all the  leaves in the subtree of $u$ that are labeled with an allocation where player $i$ wins a  bundle that contains $S$.
\end{definition}
\begin{definition}
	Fix some player $i$ and  vertex $u$ where player $i$ speaks. A bundle $S$ is \emph{decisive at price $p$} for player $i$  at the subtree of vertex $u$ if there is a strategy of player $i$ at vertex $u$ that guarantees that for every strategy profile of the other players that is consistent with vertex $u$, the protocol reaches a leaf labeled with a bundle that contains $S$ and price at most $p$.     
\shirinote{TODO - ask Shahar if it is OK to basically copy definitions from a different paper, if I cite them}
\end{definition}
\begin{theorem}
    Let $\Pi$ be an individually rational obviously-strategy proof mechanism for a combinatorial auction with general valuations with values in $\{1,2,\ldots,K=poly(m)\}$.
    Fix a node $u$ where player $i$ speaks, that has two subtrees $t_1,t_2$ with leaves $\ell_1,\ell_2$ that are labeled with 
    the allocation and payment of $(S_1,p_1)$ and $(S_2,p_2)$ respectively such that $S_1,S_2\neq \emptyset$ and $p_1,p_2<K-3$.
    \emph{Then,} both $S_1$ and $S_2$ are decisive at prices $p_1$ and $p_2$. 
    % satisfy that both $S_1$ and $S_2$ are decisive at prices at most $p_1$ and $p_2$ such that  
    % The,
    
    % satisfy that both $S_1,S_2$ are decisive at their minimal prices for player $i$ at vertex $u$.     
    % $t_1$, and $t_2$, that have to  $S_1$ 
    % it is necessarily a generalized ascending auction.     
\end{theorem}
\begin{proof}
Assume towards a contradiction that there exists a vertex $u$ 
where this does not hold \src{TODO - make this phrasing nice}. Assume that $u$ is the first vertex in the path from the root node where this condition is violated. Thus, without loss of generality, $S_1$ is not decisive at price $p_1$. 
We define the following valuation:


% If this is not true, then at least $$

% Denote the two subtrees with $t_1,t_2$ and denote the two leaves with $\ell_1,\ell_2$ and denote  their prices with $(S_1,)$
 

% Let $u$ be the highest such node in the 
\end{proof}

\subsection{Draft: Generalized Ascending Auction}
Now, to define generalized ascending auctions, two more definitions are needed. 
\begin{definition}
Fix a vertex $u$ of player $i$ and denote her set of possible messages with $Z_{i}^u$.  
 Vertex $u$ is \emph{continue-or-quit} vertex if it satisfies that if there is at most one message $z^\ast\in Z_{i}^u$ that leads to a subtree that has leaves that are labeled with non-empty bundles for player $i$. We say that message $z^\ast$ is a \emph{continue message}, and every other message in $Z_i^u$ is a \emph{quit message}.   
\end{definition}

\begin{definition}
    A \emph{generalized ascending auction} is an auction where every path admits the following structure. For every player $i$, in each node where player $i$ speaks, we have that every node satisfies 
    either all the bundles   
\end{definition}

\begin{theorem}
    Let $\Pi$ be an individually rational obviously-strategy proof mechanism for a combinatorial auction with general valuations with values in $\{1,2,\ldots,poly(m)\}$.
    Then, it is necessarily a generalized ascending auction. 
\end{theorem}

==> proof-techniques.tex <==
In this section, we explain the technical difficulties that we had to deal with when obtaining the impossibilities, which we formally prove in Sections \ref{sec-additive-unit} and \ref{sec-mua}.

\src{TODO - say that the additive and unit-demand case were more challenging to analyze, as the state of each agent given each allogcation was no longer just satisfied or not satisfied.}

\sre{Challenge 1}
One of the technical challenges in the  proofs was that we analyze at the same time
all allocation rules that give a non-trivial approximation guarantee, so we had to carefully to find valuation profiles for which we can anticipate the behavior of the mechanism that realizes them or have a sufficiently small number of plausible cases, so case analysis would be feasible.  

\sre{Challege 2}
Our work focuses on the more complex multi-parameter domains.
Due to the useful characterization that a social choice function is implementable if and only if it is monotone \cite{Mye81,AT01},  mechanism design in single-parameter domains has traditionally been simpler. For multi-parameter domains, we only have the characterization of cyclic monotonicity \cite{rochet87}, which is considerably less useful and informative. \shirinote{TODO - add weak monoticity, say that there also others}
Therefore, we do not know which social choice functions can be implemented by dominant strategy mechanisms. Naturally, this challenge persists when analyzing the more restricted class of multi-parameter social choice functions that admit obviously strategy-proof mechanisms. 
% Traditionally, mechanism design in single-parameter domains is simpler, because of the useful characterization that a social choice function is implementable if and only if it is monotone \cite{AT01,Mye81}. For multi-parameter domains, we only have the  characterization of cyclic monotonicity, which has not been very valuable so far. Thus, we do not understand well which social choice functions are implementable by dominant strategy mechanisms, and this hardness carries over to understanding which multi-parameter social choice functions satisfy the more restricted notion of being implementable by an obviously strategy-proof mechanism. 
% Therefore, the fact that our understanding of dominant-strategy mechanisms for multi-parameter domains is more limited implies that our understanding of obvious


% Thus, characterizing obviosly strategy-p
The only results for multi-parameter auctions are  the impossibility of \cite{BG17} for additive valuations and the mechanism of \cite{dKKV20} for unknown single-minded bidders in a combinatorial auction.  
% it is only known that exact welfare maximization is impossible (under normalization assumption) \cite{BG17}, and that for unknown single-minded bidders, there is an obviously-strategy proof mechanism that gives a $k$ approximation, where $k$ is the size of the largest set that a player is interested in \cite{dKKV20}.   



All of our proofs rely on the pruning technique \cite{li}, which we now describe informally. 
We begin by focusing on a set of valuations $\mathcal V=\mathcal V_1\times \cdots \times \mathcal V_n$ such that there exist $(v_1,\ldots,v_n),(v_1',\ldots,v_n')\in \mathcal V$ such that an allocation rule $f$ that gives a \textquote{good} approximation $\alpha$ outputs a different allocation for them. 
Thus, there exists some node $u$ in the mechanism where some player $i$ sends a different message for $v_i,v_i'\in \mathcal V_i$. Let $u$ be the first such node in the mechanism. The technique of pruning works by showing that the fact that player $i$ sends different messages  $m_i,m_i'$ for $v_i,v_i'$ necessarily implies that the worst case scenario given $m_i$ is less desirable for player $i$ given the valuation $v_i$ than the worst case scenario given the message $m_i'$, meaning that the mechanism is not obviously strategy-proof. See Figure \ref{figure-pruning} for an illustration. 



 
When choosing a set $\mathcal V$, we had to find a set that contains valuations that one hand are  \textquote{different} 
enough so the mechanism cannot output the same outcome for all of them, but on the other hand \textquote{similar} enough so that the best case of the mechanism given $v_i'$ will be desirable for the valuation $v_i$.




